BDD for Complete Characterization of a Safety Violation in Linear Systems with Inputs

The control design tools for linear systems typically involves pole placement and computing Lyapunov functions which are useful for ensuring stability. But given higher requirements on control design, a designer is expected to satisfy other specification such as safety or temporal logic specification as well, and a naive control design might not satisfy such specification. A control designer can employ model checking as a tool for checking safety and obtain a counterexample in case of a safety violation. While several scalable techniques for verification have been developed for safety verification of linear dynamical systems, such tools merely act as decision procedures to evaluate system safety and, consequently, yield a counterexample as an evidence to safety violation. However these model checking methods are not geared towards discovering corner cases or re-using verification artifacts for another sub-optimal safety specification. In this paper, we describe a technique for obtaining complete characterization of counterexamples for a safety violation in linear systems. The proposed technique uses the reachable set computed during safety verification for a given temporal logic formula, performs constraint propagation, and represents all modalities of counterexamples using a binary decision diagram (BDD). We introduce an approach to dynamically determine isomorphic nodes for obtaining a considerably reduced (in size) decision diagram. A thorough experimental evaluation on various benchmarks exhibits that the reduction technique achieves up to $67\%$ reduction in the number of nodes and $75\%$ reduction in the width of the decision diagram.

==> Figures/obdd-merged.tex <==
    \begin{tikzpicture}[->,shorten >=1pt,auto,node distance=1.5cm,
                    thick,main node/.style={circle,draw,font=\sffamily\small\bfseries}]

%states
 \node[state] (A) {$P^1$};
 \node[below of=A] (x11_temp) {};
 \node [state, left of=x11_temp](B1)  {$P^2$};
 \node [state, right of=x11_temp](B2)  {$P^2$};

 \node[below of=B1] (x21_temp) {};
 \node[state, left of=x21_temp] (C1) {$P^3$};
 \node[state, right of=x21_temp] (C2) {$P^3$};
 \node[below of=B2] (x22_temp) {};
 \node [state, right of=x22_temp](C3)  {$P^3$};

\node[state, below of=C1] (D1) {$P^4$};
  \node[state, below of=C2] (D2) {$P^4$};
 \node[state, below of=C3,draw=red!75,
        fill=red!20] (D3) {$P^4$};

  \node[below of=D1] (x41_temp) {};
  \node[state, right of=x41_temp,draw=red!75,
        fill=red!20] (E1) {$P^5$};
 \node[below of=D3] (x42_temp) {};
\node[state, left of=x42_temp] (E2) {$P^5$};

  \node[below of=E2] (x51_temp) {};
 \node [state, left of=x51_temp, draw=blue!75,
        fill=blue!20](T1)  {$1$};
 
%transitions
\draw (A) edge[] (B1) ;
\draw (A) edge[dashed] (B2);

\draw (B1) edge[] (C1);
\draw (B2) edge[] (C2);
\draw (B2) edge[dashed] (C3);

\draw (C1) edge[] (D1);
\draw (C1) edge[dashed] (D3);
\draw (C2) edge[] (D2);
\draw (C2) edge[dashed] (D3);
\draw (C3) edge[] (D3);
\draw (C3) edge[bend left, dashed] (D3);

\draw (D1) edge[] (E1);
\draw (D1) edge[bend right, dashed] (E1);
\draw (D2) edge[dashed] (E1);
\draw (D3) edge[dashed] (E2);

\draw (E1) edge[dashed] (T1);
\draw (E1) edge[bend right] (T1);
\draw (E2) edge[dashed] (T1);
% dotted edges
% \draw (f2) edge[bend right,dashed] (f2);
                
\end{tikzpicture}

==> Figures/obdd-original.tex <==
    \begin{tikzpicture}[->,shorten >=1pt,auto,node distance=1.5cm,
                    thick,main node/.style={circle,draw,font=\sffamily\small\bfseries}]

%states
 \node[state] (A) {$P^1$};
 \node[below of=A] (x11_temp) {};
 \node [state, left of=x11_temp](B1)  {$P^2$};
 \node [state, right of=x11_temp](B2)  {$P^2$};

 \node[below of=B1] (x21_temp) {};
 \node[state, left of=x21_temp] (C1) {$P^3$};
 \node[below of=B2] (x22_temp) {};
 \node [state, left of=x22_temp](C2)  {$P^3$};
 \node [state, right of=x22_temp](C3)  {$P^3$};

 \node[state, below of=C1] (D2) {$P^4$};
  \node[state, left of=D2] (D1) {$P^4$};
% \node[state, right of=x31_temp] (D2) {$P^4$};
 \node[below of=C2] (x31_temp) {};
  \node[state, left of=x31_temp] (D3) {$P^4$};
  \node[state, right of=x31_temp] (D4) {$P^4$};
 \node[state, below of=C3] (D5) {$P^4$};
 \node [state, right of=D5 ](D6)  {$P^4$};

%  \node [below of=D1] (x41_temp)  {};
\node[state, below of=D1] (E1) {$P^5$};
  \node[state, right of=E1] (E2) {$P^5$};
 \node [state, right of=E2] (E3)  {$P^5$};
 \node [state, right of=E3](E4)  {$P^5$};
 \node [state, below of=D4](E5)  {$P^5$};
 \node [state, below of=D5] (E6)  {$P^5$};
  \node [state, below of=D6] (E7)  {$P^5$};

  \node[below of=E4] (x51_temp) {};
 \node [state, below of=x51_temp, draw=blue!75,
        fill=blue!20](T1)  {$1$};
 
%transitions
\draw (A) edge[] (B1) ;
\draw (A) edge[dashed] (B2);

\draw (B1) edge[] (C1);
\draw (B2) edge[] (C2);
\draw (B2) edge[dashed] (C3);

\draw (C1) edge[] (D1);
\draw (C1) edge[dashed] (D2);
\draw (C2) edge[] (D3);
\draw (C2) edge[dashed] (D4);
\draw (C3) edge[] (D5);
\draw (C3) edge[dashed] (D6);

\draw (D1) edge[] (E1);
\draw (D1) edge[dashed] (E2);
\draw (D2) edge[dashed] (E3);
\draw (D3) edge[dashed] (E4);
\draw (D4) edge[dashed] (E5);
\draw (D5) edge[dashed] (E6);
\draw (D6) edge[dashed] (E7);

\draw (E1) edge[dashed] (T1);
\draw (E1) edge[bend right] (T1);
\draw (E2) edge[bend right, dashed] (T1);
\draw (E2) edge[] (T1);
\draw (E3) edge[dashed] (T1);
\draw (E4) edge[bend left] (T1);
\draw (E4) edge[dashed] (T1);
\draw (E5) edge[dashed] (T1);
\draw (E6) edge[dashed] (T1);
\draw (E7) edge[dashed] (T1);
\end{tikzpicture}



==> osc-example.tex <==
\section{Running example}

\begin{figure}
\centering     %%% not \center
% \subfigure[Without isomorphism]{\label{fig:default-bdd-basic}\includegraphics[width=0.8\linewidth]{Figures/default-bdd-basic.png}}
\subfigure[With isomorphism at level 3]{\label{fig:default-bdd-level-3}\includegraphics[width=0.6\linewidth]{Figures/default-bdd-level-3.png}}
\subfigure[With isomorphism at all levels]{\label{fig:default-bdd-all}\includegraphics[width=0.65\linewidth]{Figures/default-bdd-all.png}}
\caption{OBDD for the ordering [1, 2, 3, 4, 5].}
\label{fig:default-bdd}
\end{figure}

\begin{figure}
\centering     %%% not \center
\subfigure[Without isomorphism]{\label{fig:rev-bdd-basic}\includegraphics[width=0.8\linewidth]{Figures/rev-bdd-basic.png}}
\subfigure[With isomorphism at level 3]{\label{fig:rev-bdd-level-3}\includegraphics[width=0.6\linewidth]{Figures/rev-bdd-level-3.png}}
\subfigure[With isomorphism at all levels]{\label{fig:rev-bdd-all}\includegraphics[width=0.45\linewidth]{Figures/rev-bdd-all.png}}
\caption{OBDD for the ordering [5, 4, 3, 2, 1].}
\label{fig:rev-bdd}
\end{figure}

% \input{Figures/osc-bdd-default}
% \input{Figures/osc-bdd-rev}

==> regex-encoding.tex <==

\textbf{Problem 2} Let $L(A_r)$ is the language of a Deterministic Finite Automaton $A_r$ that expresses the regular expression $r$ over alphabet $\{0,1\}$. For a given word $\omega \in L(A_r)$, find a counterexample such that its overlapping pattern with the unsafe set conforms to $\omega$ where $\omega[i] \in \{0,1\}$ is the character at index $i$. Here, $|\omega|$ is the number of times the reachable set overlaps with the unsafe set. For instance, given the overlap interval [6 , 10] and a word  ``11010", the objective is to compute $q_0 \in \Theta$, if it exists, such that $q_6 \in U \wedge q_7 \in U \wedge q_8 \notin U \wedge q_9 \in U \wedge q_{10} \notin U$, where $q_i \deq (x_i, Loc_i) = \xi(q_0, i)$.\\

\noindent{\textbf{MILP Formulation} We introduce $|\omega|$ binary variables $z_i$. Assign $z_i = 1$ if $\omega[i] = 1$, and $z_i = 0$ otherwise. Additional $|C_i|$ binary variables $z_i^{k}$ are introduced for every set of constraints $C_i = Q_i \wedge P_i$. Each $z_i^{k}$ value is tied to a constraint in $C_i$ in such a way that any $z_i^{k} = 0$ makes the entire set $C_i$ to be unsatisfiable. We pick the parameter $\epsilon \in \mathbb{R}$ to be very small such that $0 < \epsilon < 1$. Therefore the model, for $i = 1, \ldots, |\omega|$ and $k = 1, \ldots, |C_i|$, becomes}
\begin{equation*}
\begin{aligned}
& \max \sum_{i=1}^{|\omega|} z_i \\
& \textnormal{s.t. } \left(a^{i,k}\right)^T \alpha \leq b + M \left( 1 - z_i^{k} \right), \\
&  \left(a^{i,k}\right)^T \alpha \geq b + \epsilon - M \left( z_i^{k} \right),\\
& \textnormal{ }z_i = \omega[i], \textnormal{and } z_i \leq z_i^{k}, \\
& \textnormal{ }\sum_k z_i^{k} \leq z_i + |C_i| - 1, \\
& z_i \in \{0, 1\}, z_i^{k} \in \{0, 1\}.
\end{aligned}
\end{equation*}
